Lightweight and Direct Document Relevance Optimization for Generative Information Retrieval

Generative information retrieval (GenIR) is a promising neural retrieval paradigm that formulates document retrieval as a document identifier (docid) generation task, allowing for end-to-end optimization toward a unified global retrieval objective. However, existing GenIR models suffer from token-level misalignment, where models trained to predict the next token often fail to capture document-level relevance effectively. While reinforcement learning-based methods, such as reinforcement learning from relevance feedback (RLRF), aim to address this misalignment through reward modeling, they introduce significant complexity, requiring the optimization of an auxiliary reward function followed by reinforcement fine-tuning, which is computationally expensive and often unstable. To address these challenges, we propose direct document relevance optimization (DDRO), which aligns token-level docid generation with document-level relevance estimation through direct optimization via pairwise ranking, eliminating the need for explicit reward modeling and reinforcement learning. Experimental results on benchmark datasets, including MS MARCO document and Natural Questions, show that DDRO outperforms reinforcement learning-based methods, achieving a 7.4% improvement in MRR@10 for MS MARCO and a 19.9% improvement for Natural Questions. These findings highlight DDRO's potential to enhance retrieval effectiveness with a simplified optimization approach. By framing alignment as a direct optimization problem, DDRO simplifies the ranking optimization pipeline of GenIR models while offering a viable alternative to reinforcement learning-based methods.

==> backup/exp-analysis.tex <==
% % \subsection{Result analysis}
% \begin{figure}[t]
%     \centering
%     \begin{tabular}{c}
%     \includegraphics[clip,trim=110mm 0mm 110mm 430mm,width=1.0\linewidth]{Img/retrieval_models_single_legend_readable_ENLARGED1.pdf} 
%     \\
%     \includegraphics[clip,trim=0mm 265mm 280mm 9mm,width=0.9\linewidth]{Img/retrieval_models_single_legend_readable_ENLARGED1} 
%     \\
%     (a) HITS@1 - MS MARCO
%     \\
%     \includegraphics[clip,trim=280mm 265mm 0mm 9mm,width=0.9\linewidth]{Img/retrieval_models_single_legend_readable_ENLARGED1}     
%     \\
%     (b) HITS@1 - Natural Questions
%     \\
%     \includegraphics[clip,trim=0mm 65mm 280mm 208mm,width=0.9\linewidth]{Img/retrieval_models_single_legend_readable_ENLARGED1} 
%     \\
%     (c) MRR@10 - MS MARCO
%     \\
%     FIGURE TOO LARGE
%     \\
%     (d) MRR@10 - Natural Questions
%     \if0
%     \\
%     \includegraphics[clip,trim=0mm 0mm 0mm 0mm,width=1.0\linewidth]{Img/retrieval_models_single_legend_readable_ENLARGED1} 
%     \fi
%     \end{tabular}
%     % Adjust width percentage
%     \caption{Comparison of Hits@1 and MRR@10 metrics across various retrieval models for MS MARCO and Natural Questions datasets.}
%     \Description{Comparison of the performance of various retrieval models on MS MARCO and Natural Questions datasets. The chart highlights differences in metrics such as retrieval accuracy and relevance across the models.}

%     \label{fig:performance_comparison}
% \end{figure}

% \subsection{Result analysis}



\iffalse
The experimental results \ref{tab:msmarco_nq_results} demonstrate that DDRO surpasses both traditional and generative retrieval baselines in terms of retrieval accuracy and consistency. 
On the MS MARCO dataset, DDRO (TU) achieved a Hits@1 of \textbf{38.24\%} and an MRR@10 of \textbf{50.07\%}, surpassing GenRRL (TU)of 5.23\% and 4.14\%, respectively. Similarly, on the Natural Questions dataset, DDRO (SI) achieved a Hits@1 of \textbf{48.92\%} and an MRR@10 of \textbf{55.51\%}, exceeding MINDER (SI), the closest baseline, by 8.31\% and 4.07\%.

These findings highlight that the integration of pairwise ranking with semantic and structural identifiers ensures document identifiers are generated and ranked holistically, aligning more closely with document-level relevance. This capability is particularly advantageous for knowledge-intensive queries, underscoring DDRO's potential in bridging token- and document-level gaps. Figure \ref{fig:performance_comparison} further illustrated the the performance of DDRO, compared to other baselines.
\fi


\iffalse
GenRRL\cite{zhou-etal-2023-enhancing-generative} addresses the same research question as DDRO—mitigating the over-prioritization of top-ranked results inherent in generative retrieval models. However, DDRO offers a computationally lightweight alternative by eliminating the need for reinforcement learning (RL) and reward modeling, which are resource-intensive. 
On the MS MARCO dataset, DDRO demonstrates competitive or superior performance compared to dense retrieval and other end-to-end generative retrieval models. DDRO (TU) achieves a Hits@1 of 38.24\%, significantly outperforming GenRRL (TU) at 33.01\%, demonstrating stronger top-ranked retrieval capabilities. For Hits@5, DDRO (TU) achieves 66.46\%, surpassing GenRRL (TU) at 63.62\% and aligning closely with dense retrieval models like ANCE (63.43\%). In terms of Hits@10, DDRO (TU) achieves 74.01\%, comparable to GenRRL (TU)'s 74.91\% and dense retrieval models like ANCE (74.28\%). DDRO further stands out with an MRR@10 of 50.07\%, the highest among all models, compared to 45.93\% for GenRRL (TU) and 44.09\% for ANCE, showcasing its robust ranking consistency and overall retrieval performance.

On the Natural Questions (NQ) dataset, MINDER and GenRRL exhibit strong performance in broader rankings. MINDER emerges as the strongest overall performer, achieving Hits@5 and Hits@10 scores of 65.37\% and 78.45\%, respectively, followed by GenRRL (TU) at 56.49\% and 70.96\%. DDRO (TU), with Hits@5 of 53.12\% and Hits@10 of 55.98\%, lags behind in broader rankings, reflecting a relative limitation in retrieving multiple relevant documents for NQ. However, DDRO performs well in Hits@1, achieving 40.86\% and outperforming both GenRRL (TU) at 35.79\% and MINDER at 40.61\%, underscoring its strength in identifying the most relevant document. For MRR@10, MINDER achieves the highest score of 51.44\%, followed by DDRO (TU) at 45.99\% and GenRRL (TU) at 45.73\%, highlighting MINDER’s dominance in overall ranking quality on the NQ dataset.


The ablation results in Table~\ref{tab:ablation-study} highlight the contribution of pairwise ranking optimization to DDRO's performance by enhancing retrieval quality across key metrics on both datasets.

On the MS MARCO dataset, pairwise ranking leads to notable improvements in DDRO (SI), with Hits@5 increasing from 62.62\% to 64.36\% and MRR@10 improving from 44.79\% to 45.76\%. Similarly, for DDRO (TU), Hits@5 increases from 64.60\% to 66.46\%, and MRR@10 improves from 49.18\% to 50.07\%, showcasing the role of pairwise ranking in refining overall ranking consistency and relevance distribution.

On the Natural Questions dataset, the impact of pairwise ranking is even more substantial. For DDRO (SI), Hits@5 improves from 58.44\% to 64.10\%, and MRR@10 increases from 50.48\% to 55.51\%, reflecting its importance in handling more complex queries. For DDRO (TU), Hits@5 rises from 50.50\% to 53.12\%, and MRR@10 improves from 44.32\% to 45.99\%, demonstrating its contribution to broader rankings and overall retrieval performance.

These results confirm that pairwise ranking optimization is a critical component of DDRO's architecture, driving meaningful improvements in ranking quality, particularly in broader relevance metrics, while addressing biases inherent in generative retrieval models.
\fi

\iffalse
\subsection{Identifier Design: Semantic Identifiers vs. Title+URL (RQ4)}  
Since the Docid design is an important factor, we employ different designs to evaluate the robustness of the proposed DDRO.

The findings \ref{tab:msmarco_nq_results} indicate that the effectiveness of identifier types varies across datasets. For MS MARCO, Title + URL (TU) identifiers perform well with keyword-focused queries by utilizing descriptive titles and structured URLs. In contrast, Semantic Identifiers (SI) demonstrate superior performance in Natural Questions, excelling in complex, knowledge-driven tasks by capturing latent semantic relationships beyond surface-level cues.
For example, on MS MARCO, DDRO (TU) outperformed DDRO (SI) in Hits@1 by 5.32\%, whereas on Natural Questions, DDRO (SI) surpassed DDRO (TU) by 8.06\%. These findings underline the importance of dataset alignment with identifier design.
\fi


==> backup/exp-results-table.tex <==
\begin{table*}[t]
\caption{Performance comparison across retrieval models on MS MARCO and Natural Questions (NQ). Best results are highlighted in bold. Statistical significance is determined using a paired t-test with a threshold of $p < 0.05$. Improvements are annotated as follows: $^\ast$ indicates statistically significant improvements ($p < 0.05$), while $^\dagger$ denotes non-significant improvements ($p \geq 0.05$). Abbreviations: ST -- Sparse Terms; DV -- Dense Vector; SI -- Semantic ID; NG -- N-grams; TU -- Title + URL; AT -- Atomic; Sum -- Summary.}


    \label{tab:msmarco_nq_results}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l c cccc cccc}
        \toprule
        & & \multicolumn{4}{c}{\textbf{MS MARCO}} & \multicolumn{4}{c}{\textbf{Natural Questions}} \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-10}
        \textbf{Model} & \textbf{Doc. rep/ID.} & \textbf{Hits@1} & \textbf{Hits@5} & \textbf{Hits@10} & \textbf{MRR@10} & \textbf{Hits@1} & \textbf{Hits@5} & \textbf{Hits@10} & \textbf{MRR@10} \\
        \midrule
        \multicolumn{10}{l}{\emph{Index-based retrieval}} \\
         BM25 & ST & 18.94 & 42.28 & 55.07 & 29.24 & 14.06 & 36.91 & 47.93 & 23.60 \\
        DocT5Query & ST & 23.27 & 49.38 & 63.61 & 34.81 & 19.07 & 43.88 & 55.83 & 29.55 \\
        % {SPLADE}  &   & -- & -- & -- & -- & -- & -- & -- & -- \\
        \midrule
        \multicolumn{10}{l}{\emph{Dense retrieval}} \\
        DPR & DV & 29.08 & 62.75 & 73.13 & 43.41 & 22.78 & 53.44 & 68.58 & 35.92 \\
        ANCE & DV & 29.65 & 63.43 & 74.28 & 44.09 & 24.54 & 54.21 & 69.08 & 36.88 \\
        \midrule
        \multicolumn{10}{l}{\emph{End-to-end retrieval}} \\
        DSI & SI & 25.74 & 43.58 & 53.84 & 33.92 & 27.42 & 47.26 & 56.58 & 34.31 \\
        DSI-QG & SI & 28.82 & 50.74 & 62.26 & 38.45 & 30.17 & 53.20 & 66.37 & 38.85 \\
        NCI & SI & 29.54 & 57.99 & 67.28 & 40.46 & 32.69 & 55.82 & 69.20 & 42.84 \\
        SEAL & NG & 27.58 & 52.47 & 61.01 & 37.68 & 29.30 & 54.12 & 68.53 & 40.34 \\
        
        %  {MINDER}  & SI  & -- & -- & -- & -- & -- & -- & -- & -- \\
        %  {LTRGR}  & SI  & -- & -- & -- & -- & -- & -- & -- & -- \\
        % {DGR}  & SI  & -- & -- & -- & -- & -- & -- & -- & -- \\
        % {GenRet}  & SI  & -- & -- & -- & -- & -- & -- & -- & -- \\
        % {RIPOR}  & SI  & -- & -- & -- & -- & -- & -- & -- & -- \\
        % {PAG}  & SI  & -- & -- & -- & -- & -- & -- & -- & -- \\
        
        Ultron   & SI & 32.18 & 62.00 & 69.55 & 44.57 & 31.12 & 43.90 & 48.16 & 36.65 \\
        Ultron  & TU & 38.49 & 65.22 & 72.15 & 49.50& 33.63 & 46.06 & 49.62 & 38.98 \\
        SFT~\cite{zhou-etal-2023-enhancing-generative} & TU & 29.90 & 60.28 & 68.17 & 42.52 & 33.91 & 54.18 & 66.92 & 42.52 \\
        GenRRL~\cite{zhou-etal-2023-enhancing-generative} & TU & 33.01 & 63.62 & 74.91 & 45.93 & 35.79 & 56.49 & 70.96 & 45.73 \\
        \midrule
        \multicolumn{10}{l}{\emph{Ours}} \\
        {SFT} & SI   & 32.18 & 62.62 & 71.29 &44.79 & 44.19 & 58.44 & 62.23 & 50.48 \\
        {SFT} & TU & 38.12 & 64.60 &72.90& 49.18 &  39.58 & 50.50 & 53.53 & 44.32 \\

         {DDRO} & SI & 32.92 & 64.36 & 73.02 & 45.76 &  {48.92}  & {64.10}  & {67.31} & {55.51} \\
        {DDRO} & TU & 38.24 &66.46 & 74.01& 50.07 &   40.86 & 53.12& 55.98 & 45.99 \\
        \bottomrule
\end{tabular}}
\end{table*}


==> backup/result-discussion.tex <==
\iffalse
\subsection{Result discussion}
While DDRO slightly lags behind GenRRL in broader rankings, such as Hits@5 and Hits@10 on the Natural Questions dataset, this can be attributed to its emphasis on computational efficiency and simpler approach to relevance alignment at the document level. In contrast, GenRRL employs a more sophisticated approach, incorporating reinforcement learning with reward modeling and listwise ranking optimization.  GenRRL employs a more sophisticated approach, incorporating reinforcement learning with reward modeling and listwise ranking optimization. These techniques allow GenRRL to better capture relationships across multiple relevant documents, leading to superior performance in broader rankings. However, DDRO’s trade-offs make it more scalable and cost-effective for resource-constrained scenarios. To mitigate these limitations, future work could explore integrating listwise ranking objectives or dynamic identifier selection methods to better address complex, knowledge-driven queries in datasets like NQ. Additionally, adopting hybrid strategies that combine semantic identifiers with hard negative mining could enhance the retrieval of mid-ranked documents, improving broader rankings without compromising efficiency.
This distinction between DDRO and GenRRL’s performance can also be observed when comparing the effectiveness of Title + URL (TU) and Semantic Identifiers (SI) across datasets, as these identifiers play a pivotal role in determining retrieval outcomes.


\textbf{Nature of the Datasets:}
 MS MARCO focuses on web pages, where Title + URL (TU) naturally provide valuable signals. Titles in web search results are typically crafted to be descriptive, closely aligning with user search intent, while URLs often contain structured tokens, such as keywords or domains, that are highly indicative of relevance for web-based queries. In contrast, Natural Questions (NQ), being Wikipedia-based, features factual, knowledge-dense documents. Titles and URLs on Wikipedia are more uniform and less informative as surface-level signals, limiting their utility. In this context, Semantic Identifiers (SI), generated through methods like product quantization or clustering, excel at capturing deeper semantic relationships within the content, aligning more effectively with the query-driven and knowledge-seeking nature of NQ.


 
\textbf{Query Types:}
 MS MARCO queries, derived from real-world web search logs, encompass a mix of informational, navigational, and transactional intents. These queries are often shorter and keyword-focused, resembling web search behavior, where surface-level signals in titles and URLs align well with user intent and relevance labels. This makes TU particularly effective for MS MARCO tasks. In contrast, NQ queries are predominantly informational and more complex, often framed as longer questions requiring deeper semantic understanding for accurate retrieval.

 
\textbf{Document Structure:}
 In web documents within MS MARCO, titles and URLs frequently serve as concise, descriptive summaries of content, aligning closely with keyword-driven queries and making TU a highly effective identifier. In these contexts, deeper semantic encodings like SI may offer limited additional benefit over surface-level lexical signals. Conversely, in Wikipedia documents from Natural Questions (NQ), leading sentences or abstracts often do not directly match query terms, and titles and URLs provide minimal relevance cues. Here, SI, which captures latent semantic relationships, better reflects the overall document meaning and aligns more effectively with the query, particularly for complex, knowledge-seeking tasks.

 
\textbf{Training Dynamics:}
 Models trained on MS MARCO tend to rely heavily on surface-level lexical features, such as titles and URLs, which align well with short, keyword-based matches common in web search queries. This reliance can lead to overfitting when the dataset rewards structured identifiers. In contrast, Natural Questions (NQ), with its longer passages and factual, knowledge-rich content, requires models to generalize more deeply. Here, Semantic Identifiers (SI) demonstrate their strength by capturing latent semantic relationships that align more effectively with complex, informational queries.
 
In summary, the superior performance of TU on MS MARCO stems from its ability to exploit surface-level matches provided by structured identifiers like titles and URLs, which are well-suited for web-based, keyword-driven queries. On the other hand, SI outperforms on NQ due to its capacity to capture deeper semantic meanings, essential for addressing complex, informational queries in factual, knowledge-heavy documents. This distinction underscores the importance of aligning representation methods with the specific characteristics of datasets and their respective tasks. These findings also validate DDRO’s flexibility in leveraging identifier strategies to meet dataset-specific requirements, while emphasizing the potential for future improvements to address broader ranking limitations.
 \fi



==> sections/direct-document-relevance-optimization.tex <==
\section{Direct Document Relevance Optimization (DDRO)}
Inspired by \cite{Rafailov2023DirectPO} we propose Direct Document Relevance Optimization (DDRO). DDRO is a single-stage alignment algorithm used to fine-tune large language models (LLMs). This method avoids the need for reinforcement learning or a separate reward model. Instead, it reparameterizes the reward function, enabling the extraction of the optimal policy in closed form by treating it as a simple classification problem on the relevance pairs \cite{Rafailov2023DirectPO}. DDRO provides better control over the model's outputs, demonstrating a superior ability to guide generation toward relevant results \cite{Rafailov2023DirectPO}.

DDRO optimizes the same objective as Reinforcement Learning from Relevance Feedback (RLRF) \cite{zhou-etal-2023-enhancing-generative, Christiano2017DeepRL, Bai2022ConstitutionalAH, Stiennon2020LearningTS, Nakano2021WebGPTBQ, Li2023ReinforcementLW, Ouyang2022TrainingLM, Christiano2017DeepRL}, aiming to maximize rewards while maintaining alignment with human preferences via a KL divergence constraint. RLRF achieves this by using a learned reward function to refine language model outputs, as formalized in previous work \cite{Jaques2016SequenceTC, Jaques2020HumancentricDT}.
%
\begin{equation}
\max_{\pi_\theta} \mathbb{E}_{x \sim \mathcal{D}, y \sim \pi_\theta(y|x)} \left[ r_\phi(x, y) \right] - \beta \mathbb{D}_{\text{KL}}\left( \pi_\theta(y | x) \| \pi^{\text{ref}}(y | x) \right),
\end{equation}
%
where \( \beta \) controls the divergence from the reference policy \( \pi^{\text{ref}} \), which is typically the initially pre-trained model. This constraint prevents the model from straying too far from the data distribution used to train the reward function, preserving output diversity and avoiding overfitting to high-reward responses. Since language generation is non-differentiable, reinforcement learning techniques are widely used. A widely recognized approach \cite{Ziegler2019FineTuningLM, Stiennon2020LearningTS, Ouyang2022TrainingLM} optimizes the reward function using Proximal Policy Optimization (PPO) \cite{Schulman2017ProximalPO}, and defines the reward function as:
%
\begin{equation}
r(x, y) = r_\phi(x, y) - \beta (\log \pi_\theta(y | x) - \log \pi^{\text{ref}}(y | x)).
\end{equation} 
%



In contrast to RLHF, DDRO bypasses the need for modeling a reward function and applying reinforcement learning. Instead, DDRO directly maximizes the likelihood that relevant documents ($d^+$) receive higher scores than non-relevant ones ($d^-$) for a given query. The corresponding optimization objective is formulated as:
%
\begin{equation}
\begin{split}
&\mathcal{L}_{\text{DDRO}}(\pi_{\theta};\pi^{\text{ref}}) = {}\\
& -\mathbb{E}_{(q, \bm{d}^+, \bm{d}^-) \sim D} \left[ 
    \log \sigma \left( \beta \log \frac{\pi_{\theta}(\bm{d}^+ \mid q)}{\pi^{\text{ref}}(\bm{d}^+ \mid q)}
    - \beta \log \frac{\pi_{\theta}(\bm{d}^- \mid q)}{\pi^{\text{ref}}(\bm{d}^- \mid q)} \right) 
    \right],
\end{split}    
\end{equation}
%
where  \( \pi_\theta(d | q) \) is the policy being optimized, and \( \pi^{\text{ref}}(d | q) \) is the reference policy, typically the fine-tuned model (SFT model). This formulation ensures that the model stays close to the reference policy while still optimizing for relevance-based responses. The DDRO update efficiently guides the model toward producing outputs better aligned with relevance by utilizing pairwise comparisons, offering a more effective alternative to  RL-based methods. The gradient with respect to the model parameters $\theta$ is defined as:
%
\begin{multline}
\nabla_\theta \mathcal{L}_{\mathrm{DDRO}}\left(\pi_\theta ; \pi^{\text{ref}}\right) = \\
-\beta \mathbb{E}_{\left(q, d^+, d^-\right) \sim \mathcal{D}}[\underbrace{\sigma\left(\hat{r}_\theta\left(q, d^-\right)-\hat{r}_\theta\left(q, d^+\right)\right)}_{\text {higher weight when reward estimate is wrong }} \times \\
[\underbrace{\nabla_\theta \log \pi\left(d^+ \mid q\right)}_{\text {increase likelihood of } d^+} - \underbrace{\nabla_\theta \log \pi\left(d^- \mid q\right)}_{\text {decrease likelihood of } d^-}]],
\end{multline}
%
where \( \hat{r}_\theta(q, d) = \beta \log \frac{\pi_\theta(d \mid q)}{\pi^{\text{ref}}(d \mid q)} \) is the reward implicitly defined by the language model \( \pi_\theta \) and the reference model \( \pi^{\text{ref}} \). The examples are weighted according to how much the implicit reward model \( \hat{r}_\theta \) overestimates the ranking of the non-relevant document \( d^- \) compared to the relevant document \( d^+ \). This weighting is scaled by \( \beta \), reflecting the degree of misjudgment while considering the strength of the KL divergence constraint. The sigmoid function \( \sigma(\cdot) \) ensures smooth optimization, and the model parameters \( \theta \) are adjusted to increase the likelihood of the relevant document \( d^+ \) while decreasing the likelihood of the non-relevant document \( d^- \). This reparameterization reduces the need for complex reward models and iterative fine-tuning, making DDRO a more scalable and stable alternative for aligning large language models with document-level relevance tasks.


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Img/workflow.pdf} 
    \caption{\textcolor{blue}{The overview workflow includes three steps: (1) We construct three types of DocIDs, i.e., URL / title and domain, leading sentences, and product quantization codes; (2) based on the constructed DocIDs, we initially perform supervised fine-tuning of the retrieval model $\pi_\theta^{ref}$ with multiple types of data pairs; and (3) we freeze the trained model $\pi_\theta^{ref}$ as the reference model and further perform L2R optimization on a policy model $\pi_\theta$ using DDRO.}} 
    \label{fig:workflow}
\end{figure*}


